Learning Bermudans

American and Bermudan-type financial instruments are often priced with specific Monte Carlo techniques whose efficiency critically depends on the effective dimensionality of the problem and the available computational power. In our work we focus on Bermudan Swaptions, well-known interest rate derivatives embedded in callable debt instruments or traded in the OTC market for hedging or speculation purposes, and we adopt an original pricing approach based on Supervised Learning (SL) algorithms. In particular, we link the price of a Bermudan Swaption to its natural hedges, i.e. the underlying European Swaptions, and other sound financial quantities through SL non-parametric regressions. We test different algorithms, from linear models to decision tree-based models and Artificial Neural Networks (ANN), analyzing their predictive performances. All the SL algorithms result to be reliable and fast, allowing to overcome the computational bottleneck of standard Monte Carlo simulations; the best performing algorithms for our problem result to be Ridge, ANN and Gradient Boosted Regression Tree. Moreover, using feature importance techniques, we are able to rank the most important driving factors of a Bermudan Swaption price, confirming that the value of the maximum underlying European Swaption is the prevailing feature.

==> Learning Bermudans/Newcommands.tex <==
% --- Definitions of new Latex commands ---
%
% REMIND: always keep a single file with all definitions, beware of multiple copies.

% --- Text ---
\newcommand{\ie}{i.e.~} 	                    % i.e. with non-breakable space
\newcommand{\eg}{e.g.~} 	                    % e.g. with non-breakable space
\newcommand{\rhs}{r.h.s.~} 	                    % r.h.s. with non-breakable space
\newcommand{\wrt}{w.r.t.~} 	                    % w.r.t. with non-breakable space
\newcommand{\old}[1]{\textcolor{blue}{#1}}      % old text, blue, strike-through tex
\newcommand{\new}[1]{\textcolor{red}{#1}}       % new text, red, strike-through tex
%\newcommand{\comment}[1]{\textcolor{green}{#1}} % comments, green, strike-through tex
\newcommand{\textbox}[1]{\mbox{\textit{#1}}} 	% text inside math
\newcommand{\virgolette}[1]{``#1''}

% --- Mathematical Definitions ---
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{definitions}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}[theorem]{Example}
\newtheorem{lemma}[theorem]{Lemma}

% --- Environments ---
\newenvironment{system}{\left\lbrace\begin{array}{@{}l@{}}}{\end{array}\right.}

% --- Delimiters ---
\newcommand{\Parenthesis}[1]{\left( #1 \right)}         % (xxx)
\newcommand{\Brack}[1]{\left\lbrack #1 \right\rbrack}   % [xxx]
\newcommand{\Brace}[1]{\left\lbrace #1 \right\rbrace}   % {xxx}
\newcommand{\Abs}[1]{\left\lvert #1 \right\rvert}       % |xxx|
\newcommand{\Norm}[1]{\left\lVert #1 \right\rVert}      % ||xxx||
\newcommand{\Mean}[1]{\left\langle #1 \right\rangle}    % <xxx>
\newcommand{\QuoteDouble}[1]{``#1''}                    % double quotation marks
\newcommand{\QuoteSingle}[1]{`#1'}                      % single quotation marks

% --- Math operators ---
\newcommand{\beq}{\begin{equation}}         % \begin{equation}
\newcommand{\eeq}{\end{equation}}           % \end{equation}
\newcommand{\Max}{\mbox{Max}}                                   % Max operator
\newcommand{\Min}{\mbox{Min}}                                   % Min operator
\newcommand{\Derp}[2]{\frac{\partial #1}{\partial #2}}          % partial derivative, 1st order
\newcommand{\DerpXX}[2]{\frac{\partial^2 #1}{\partial #2 ^2}}   % partial derivative, 2nd order
\newcommand{\DerpXY}[3]{\frac{\partial^2 #1}{\partial #2 \partial #3}}    % partial derivative, 2nd order, cross
\newcommand{\half}[0]{\frac{1}{2}}                                                  % one half
\newcommand{\ind}[1]{\mathbf{1}_{#1}} 	                                            % indicator
\newcommand{\E}[1]{\mathbb{E}\left[#1\right]}                                       % Expected value
\newcommand{\expt}[1]{\mathbb{E}_t\left[#1\right]}                                  % Expected value at time t
\newcommand{\Econd}[2]{\mathbb{E}\left[#1\;\middle \vert\;\mathcal{F}_{#2}\right]}  % Expected value conditioned

% --- Sets ---
\newcommand{\Nset}{\mathbb{N}}      % Natural numbers set
\newcommand{\Zset}{\mathbb{Z}}      % Integer numbers set
\newcommand{\Qset}{\mathbb{Q}}      % Rational numbers set
\newcommand{\Rset}{\mathbb{R}}      % Real numbers set

% --- Finance ---
\newcommand{\Black}{\mbox{Black}}				    % Black's formula
\newcommand{\XVA}{\mbox{\textit{XVA}}}				% XVA
\newcommand{\CVA}{\mbox{\textit{CVA}}}				% CVA
\newcommand{\DVA}{\mbox{\textit{DVA}}}				% DVA
\newcommand{\FVA}{\mbox{\textit{FVA}}}				% FVA

% --- Financial Instruments ---
\newcommand{\Depo}{\mbox{\textbf{Depo}}}			% Deposit
\newcommand{\FRA}{\mbox{\textbf{FRA}}}			    % Forward Rate Agreement
\newcommand{\Futures}{\mbox{\textbf{Futures}}}      % Futures
\newcommand{\ZCB}{\mbox{ZCB}}					    % Zero Coupon Bond
\newcommand{\Swap}{\mbox{\textbf{Swap}}}			% Swap
\newcommand{\Swaplet}{\mbox{\textbf{Swaplet}}}		% Swaplet
\newcommand{\IRS}{\mbox{\textbf{IRS}}}			    % Interest Rate Swap
\newcommand{\IRSlet}{\mbox{\textbf{IRSlet}}}        % Interest Rate Swaplet
\newcommand{\OIS}{\mbox{\textbf{OIS}}}              % OIS (Overnight Indexed Swap)
\newcommand{\OISlet}{\mbox{\textbf{OISlet}}}        % OISlet
\newcommand{\BSwap}{\mbox{\textbf{BSwap}}}          % Basis Swap
\newcommand{\BSwaplet}{\mbox{\textbf{BSwaplet}}}    % Basis Swaplet
\newcommand{\IRBS}{\mbox{\textbf{IRBS}}}            % Interest Rate Basis Swap
\newcommand{\IRBSlet}{\mbox{\textbf{IRBSlet}}}      % Interest Rate Basis Swaplet
\newcommand{\CCSwap}{\mbox{\textbf{CCSwap}}}        % Cross Currency Swap
\newcommand{\CCS}{\mbox{\textbf{CCS}}}              % Cross Currency Swap
\newcommand{\CCSwaplet}{\mbox{\textbf{CCSwaplet}}}  % Cross Currency Swaplet
\newcommand{\CCSlet}{\mbox{\textbf{CCSlet}}}        % Cross Currency Swaplet
\newcommand{\Caplet}{\mbox{\textbf{Caplet}}}        % Caplet
\newcommand{\Floorlet}{\mbox{\textbf{Floorlet}}}    % Floorlet
\newcommand{\cf}{\mbox{\textbf{cf}}}                % Caplet/Floorlet
\newcommand{\CAP}{\mbox{\textbf{Cap}}}              % Cap
\newcommand{\Floor}{\mbox{\textbf{Floor}}}          % Floor
\newcommand{\CF}{\mbox{\textbf{CF}}}                % Cap/Floor
\newcommand{\Swaption}{\mbox{\textbf{Swaption}}}    % Swaption
\newcommand{\CMSlet}{\mbox{\textbf{CMSlet}}}        % CMSlet
\newcommand{\CMS}{\mbox{\textbf{CMS}}}              % CMS
\newcommand{\CMScf}{\mbox{\textbf{CMScf}}}          % CMS caplet/floorlet
\newcommand{\FXFwd}{\mbox{\textbf{FXFwd}}}          % Forex forward
%\newcommand{\FP}{\mbox{FP}}
%\newcommand{\CB}{\mbox{ CB}}
%\newcommand{\Bl}{\mbox{Bl}}
%\newcommand{\ZBC}{\mbox{ ZBC}}
%\newcommand{\ZBP}{\mbox{ ZBP}}
%\newcommand{\ZBO}{\mbox{ ZBO}}
%\newcommand{\CBC}{\mbox{ CBC}}
%\newcommand{\CBP}{\mbox{ CBP}}
%\newcommand{\CBO}{\mbox{ CBO}}
%\newcommand{\FSCpl}{\mbox{ FSCpl}}
%\newcommand{\Fll}{\mbox{ Fll}}
%\newcommand{\PFS}{\mbox{ PFS}}
%\newcommand{\RFS}{\mbox{ RFS}}
%\newcommand{\PS}{\mbox{ PS}}
%\newcommand{\PBS}{\mbox{ PBS}}
%\newcommand{\RS}{\mbox{ RS}}
%\newcommand{\ES}{\mbox{ ES}}
%\newcommand{\Var}{\mbox{Var}}
%\newcommand{\Cov}{\mbox{Cov}}
%\newcommand{\Std}{\mbox{Std}}
%\newcommand{\Corr}{\mbox{Corr}}
%\newcommand{\QCap}{\mbox{ QCap}}
%\newcommand{\QFlr}{\mbox{ QFlr}}
%\newcommand{\QCpl}{\mbox{ QCpl}}
%\newcommand{\QFll}{\mbox{ QFll}}
%\newcommand{\QS}{\mbox{ QS}}
%\newcommand{\QES}{\mbox{ QES}}
%\newcommand{\LSO}{\mbox{ LSO}}
%\newcommand{\LP}{\mbox{ LP}}
%\newcommand{\TSD}{\mbox{ TSD}}
%\newcommand{\TSF}{\mbox{ TSF}}
%\newcommand{\pftd}{\Pi\mbox{\tiny RFtD}}
%\newcommand{\ftd}{\mbox{FtD}}


% --- Credit new commands ---
%\newcommand{\gtrapprox}{> \approx}
%\newcommand{\op}{\mbox{OP}}
%\newcommand{\swp}{\PS}
%\newcommand{\Qt}{\mathbb{Q}_t}
%\newcommand{\indle}{\textbf{1}_{\{\tau\leq T\}}}
%\newcommand{\indg}{\textbf{1}_{\{\tau >T\}}}
%\newcommand{\indgt}{\textbf{1}_{\{\tau >t\}}}
%\newcommand{\cash}{\mbox{C{\tiny ASHFLOW}}}
%\newcommand {\Sund} {\underline{S}}
%\newcommand {\xund} {\underline{x}}
%\newcommand{\cds}{\mbox{CDS}}
%\newcommand{\Ex}{\Bbb{E}}
%\newcommand{\Qx}{\Bbb{Q}}
%\newcommand{\Px}{\Bbb{P}}
%\newcommand{\gamimpl}{\gamma^{\mbox{\tiny mkt}}}
%\newcommand{\Gamimpl}{\Gamma^{\mbox{\tiny mkt}}}
%\newcommand{\pracds}{\mbox{PR2CDS}}
%\newcommand{\Mkt}{\tiny \mbox{Mkt}}
%\newcommand{\prcds}{\mbox{PRCDS}}
%\newcommand{\cdo}{\mbox{CDO}}
%\newcommand{\cdoi}{\mbox{CDOin}}
%\newcommand{\cdotr}{\mbox{CDOtr}}
%\newcommand{\cdosq}{\mbox{CDOsq}}
%\newcommand{\cmcds}{\mbox{CDScm}}
%\newcommand{\Rtil}{\widetilde{R}}
%\newcommand{\Lsq}{{\cal L}}
%\newcommand{\ucds}{\mbox{UCDS}}
%\newcommand{\vsp}{\vspace{1cm}}
%\newcommand{\vsh}{\vspace{0.5cm}}
%\newcommand{\hsp}{\hspace{0.5cm}}
%\newcommand{\sbar}{\nu}
%\newcommand{\F}{\cal F}
%\newcommand{\sigb}{\bar{\sigma}}
%\newcommand{\nub}{\bar{\sbar}}
%\newcommand{\trace}{{\rm trace}}
%\newcommand{\rank}{{\rm rank}}
%\newcommand{\threequarter}{{\textstyle\frac{3}{4}}}
%\newcommand{\ppit}{{\displaystyle p_t^\pi}}
%\newcommand{\barF}{\bar{F}}
%\newcommand{\barP}{\bar{P}}
%\newcommand{\lgd}{\mbox{L{\tiny GD}}}
%\newcommand{\rec}{\mbox{R{\tiny EC}}}
%\newcommand{\pcds}{\Pi\mbox{\tiny RCDS}}
%\newcommand{\pprcds}{\Pi\mbox{\tiny PRCDS}}
%\newcommand{\pcdo}{\Pi\mbox{\tiny CDO}}
%\newcommand{\pcdosq}{\Pi\mbox{\tiny CDOSQ}}
%\newcommand{\ppracds}{\Pi\mbox{\tiny PR2CDS}}
%\newcommand{\pucds}{\Pi\mbox{\tiny UCDS}}
%\newcommand{\ppucds}{\Pi\mbox{\tiny UPCDS}}
%\newcommand{\pdfrn}{\Pi\mbox{\tiny DFRN}}
%\newcommand{\pdfrna}{\Pi\mbox{\tiny DFRN1}}
%\newcommand{\pdfrnb}{\Pi\mbox{\tiny DFRN2}}
%\newcommand{\pccds}{\Pi\mbox{\tiny CallCDS}}
%\newcommand{\ppcds}{\Pi\mbox{\tiny PutCDS}}
%\newcommand{\pcprcds}{\Pi\mbox{\tiny CallPRCDS}}
%\newcommand{\ppprcds}{\Pi\mbox{\tiny PutPRCDS}}
%\newcommand{\pcpracds}{\Pi\mbox{\tiny CallPR2CDS}}
%\newcommand{\pppracds}{\Pi\mbox{\tiny PutPR2CDS}}
%\newcommand{\dfrn}{\mbox{DFRN}}
%\newcommand{\dfrna}{\mbox{DFRN1}}
%\newcommand{\dfrnb}{\mbox{DFRN2}}
%\newcommand{\ccds}{\mbox{CallCDS}}
%\newcommand{\cprcds}{\mbox{CallPRCDS}}
%\renewcommand{\H}{{\scriptstyle H}}
%\newcommand{\dib}{\mbox{DIB}}
%\newcommand{\dob}{\mbox{DOB}}
%\newcommand{\Ctil}{\widetilde{C}}
%\newcommand{\ctil}{\tilde{c}}
%\newcommand{\chat}{\widehat{c}}
%\newcommand{\cbar}{\bar{c}}
%\newcommand{\Cbar}{\bar{C}}
%\newcommand{\cbarhat}{\widehat{\bar{c}}}
%\newcommand{\Cbarhat}{\widehat{\bar{C}}}
%\newcommand{\npvv}{\overline{\mbox{NPV}}}
%\newcommand{\npv}{\mbox{NPV}}
%\newcommand{\defree}{\mbox{\tiny DEFREE}}
%\newcommand{\taub}{\tau_{B}}
%\newcommand{\tauc}{\tau_{C}}
%\newcommand{\Hhat}{\widehat{H}}
%\newcommand{\xcn}{\tilde{x}^{\alpha}}
%\newcommand{\pas}{\frac{T}{n}}
%\newcommand{\past}{(t_{i+1}-t_i)}
%\newcommand{\pasW}{(W_{t_{i+1}}-W_{t_i})}
%\newcommand{\GO}{\mathcal{O}}
%\newcommand{\F}{\mathcal{F}}
%\newcommand{\HS}{\mathcal{H}_S}
%\newcommand{\HW}{\mathcal{H}_W}
%\newcommand{\zb}{\bar{z}}
%\newcommand{\dM}{\dot{M}}
%\newcommand{\swp}{\PS}

